Poisoning $\times$ Evasion: Symbiotic Adversarial Robustness for Graph Neural Networks

It is well-known that deep learning models are vulnerable to small input perturbations. Such perturbed instances are called adversarial examples. Adversarial examples are commonly crafted to fool a model either at training time (poisoning) or test time (evasion). In this work, we study the symbiosis of poisoning and evasion. We show that combining both threat models can substantially improve the devastating efficacy of adversarial attacks. Specifically, we study the robustness of Graph Neural Networks (GNNs) under structure perturbations and devise a memory-efficient adaptive end-to-end attack for the novel threat model using first-order optimization.

==> tables/jaccard.tex <==
\begin{table}[t!]
    \centering
    \caption{Average (± standard error) perturbed accuracies for the evasion, poisoning, symbiotic attacks over 10 runs with a 5\% budget on the graphs pre-processed with \textbf{Jaccard purification} \citep{wuAdversarialExamplesGraph2019}. The strongest attacks for each setup are written in bold.}
    \label{tab:jaccard}
    \begin{tabular}{llllll}
        \toprule
        \textbf{Dataset} & \textbf{Model} & \textbf{Clean} & \textbf{Evasion} & \textbf{Poisoning} & \textbf{Symbiotic} \\
        \midrule
        \multirow[t]{5}{*}{CiteSeer} 
         & GCN & 0.68 ± 0.01 & 0.41 ± 0.01 & 0.41 ± 0.02 & \textbf{0.38 ± 0.01} \\
         & GAT & 0.64 ± 0.01 & 0.32 ± 0.03 & 0.41 ± 0.03 & \textbf{0.3 ± 0.03} \\
         & APPNP & 0.68 ± 0.01 & \textbf{0.43 ± 0.01} & 0.52 ± 0.02 & 0.45 ± 0.02 \\
         & GPRGNN & 0.65 ± 0.01 & \textbf{0.35 ± 0.01} & 0.44 ± 0.01 & \textbf{0.35 ± 0.01}\\
        \midrule
        \multirow[t]{5}{*}{Cora} 
         & GCN & 0.74 ± 0.01 & 0.39 ± 0.01 & 0.43 ± 0.02 & \textbf{0.36 ± 0.01} \\
         & GAT & 0.67 ± 0.01 & \textbf{0.23 ± 0.02} & 0.45 ± 0.02 & 0.28 ± 0.02 \\
         & APPNP & 0.82 ± 0.01 & \textbf{0.5 ± 0.01} & 0.67 ± 0.01 & 0.54 ± 0.01 \\
         & GPRGNN & 0.79 ± 0.01 & 0.44 ± 0.01 & 0.54 ± 0.01 & \textbf{0.4 ± 0.01} \\
        \midrule
        \multirow[t]{5}{*}{PubMed} 
         & GCN & 0.77 ± 0.01 & 0.41 ± 0.01 & 0.11 ± 0.01 & \textbf{0.02 ± 0.0} \\
         & GAT & 0.74 ± 0.01 & 0.34 ± 0.04 & 0.38 ± 0.04 & \textbf{0.19 ± 0.02} \\
         & APPNP & 0.77 ± 0.01 & 0.45 ± 0.01 & 0.19 ± 0.03 & \textbf{0.1 ± 0.02} \\
         & GPRGNN & 0.78 ± 0.01 & 0.42 ± 0.01 & 0.38 ± 0.04 & \textbf{0.15 ± 0.04} \\
        \bottomrule
    \end{tabular}
\end{table}
